"What Keeps People Secure is That They Met The Security Team": Deconstructing Drivers And Goals of Organizational Security Awareness

Security awareness campaigns in organizations now collectively cost billions of dollars annually. There is increasing focus on ensuring certain security behaviors among employees. On the surface, this would imply a user-centered view of security in organizations. Despite this, the basis of what security awareness managers do and what decides this are unclear. We conducted n=15 semi-structured interviews with full-time security awareness managers, with experience across various national and international companies in European countries, with thousands of employees. Through thematic analysis, we identify that success in awareness management is fragile while having the potential to improve; there are a range of restrictions, and mismatched drivers and goals for security awareness, affecting how it is structured, delivered, measured, and improved. We find that security awareness as a practice is underspecified, and split between messaging around secure behaviors and connecting to employees, with a lack of recognition for the measures that awareness managers regard as important. We discuss ways forward, including alternative indicators of success, and security usability advocacy for employees.

==> assets/codebook.tex <==
\onecolumn

%\newcolumntype{s}{>{\hsize=.0.5\hsize}X}
\section*{Code Book For The Paper \enquote{'What Keeps People Secure is That They Met The Security Team':
Deconstructing Drivers And Goals of Organizational Security Awareness} \\ {\small by Jonas Hielscher, Ruhr University Bochum \& Simon Parkin, Delft University of Technology}}
\label{app:codebook}

\begin{table*}[!ht]
\small
\centering
\caption{Our code book with main categories (bold) -- 1/2.}
\label{app:tab:code1}
\begin{tabular}{p{3cm}p{5cm}p{5cm}p{1cm}r}
\rowcolor[HTML]{EFEFEF} 
\hline
\hline
\textbf{Code}        & \textbf{Description}   & \textbf{Example Quote} & \textbf{Section} & \textbf{Count}                                       \\ \hline
\textbf{Awareness in Organization} & & & & \\                                     

\rowcolor[HTML]{EFEFEF} Influence on Content and Activity & What does influence the content of the awareness products or the decision on what products are used (\eg, attacks, pressure from the news, the employees, the management) & So we went through a bit of an exercise previously where we kind of went through all of our training. And we said, have we had any incidents involving any of these topics? And if we haven't, then we scrapped it. (P15) & 
4.2.3
%\ref{results:whatInformsAwareness} 
&  54 \\        

Vendor & Which vendors are involved in the awareness activities in the participants' organization and how? & But it's still product-led. It's still in the sense that when you get a team in, head of awareness or similar type of, they will typically look to go, what product can I get to help me with? That's a problem. (P13) & 
4.4.1
%\ref{results:vendors} 
& 66 \\

\rowcolor[HTML]{EFEFEF} Success/Goal & What makes a successful security awareness for the participant/ for the organization. And more general: What is the goal of awareness for the organization? & The assets of training and what have you are a thing that is needed, because that's what people say that you need to train people, to give them knowledge. But realistically I don't know really how well that works and it's really hard to gauge how well it actually works in practice. (P19) & 
4.3.1, 4.3.2
%\ref{results:goal}, \ref{results:measuring}
& 54\\

Activities & Enumeration of awareness activities (\eg, phishing simulation, gamification, town halls, online training, etc.) & the e-training to practice to put, I have completely renewed last year, central and that goes only nineteen minutes and there are all the topics in it (P5) & 
4.2.1
%\ref{results:activities} 
& 158 \\

\rowcolor[HTML]{EFEFEF} Metrics/Measurements & How is the success of awareness (not) measured? & So making an evaluation of how many Prada bags I could afford from your click errors. I'm sure that would have an impressive impact. But I think I might have a problem with compliance. (P7) & 
4.3.2
%\ref{results:measuring}
& 91\\

Regulation/Norms/External Forces &How do regulations (ISO27001, etc.) influence the security awareness in the organization? & That's the easy way to do it, via the online tool. To say the auditors are asking for it that way. So even if we say we do all face-to-face, it will be difficult to get it through. It's just much easier to check online. (P1) & 
4.4.2
%\ref{results:regulations} 
& 91\\

\rowcolor[HTML]{EFEFEF} \textbf{Bad Practices Persist} & What or who keeps bad awareness practices persisting and why? &So his and that is very common, particularly in this country is, that people get their understanding from what vendors say. And it's almost like the cool kids in the classroom, you know, a viral on social media. If there are enough people saying it, it's like the emperors' new clothes. (P11) & 
4.4.1, 4.3.2
%\ref{results:vendors}, \ref{results:measuring} 
& 144 \\

\textbf{Employees} &-&-&-&-\\

\rowcolor[HTML]{EFEFEF} Perception of Employees & How do the participants describe employees, their attitude, their security behavior, how do they perceive them? &And then you get questions like, "What is multifactor authentication?" And then you just think to yourself, "Oh great, they didn't get anything." (P2) & 
4.6
%\ref{sec:res:employees} 
& 31 \\


\hline\hline
\end{tabular}
\end{table*}


\begin{table*}[!ht]
\small
\centering
\caption{Our code book with main categories (bold) -- 2/2.}
\label{app:tab:code2}
\begin{tabular}{p{3cm}p{5cm}p{5cm}p{1cm}r}
\hline
\hline
\rowcolor[HTML]{EFEFEF}\textbf{Code}        & \textbf{Description}   & \textbf{Example Quote} & \textbf{Section} & \textbf{Count}                                       \\ \hline                               
Communication \& Relationship & (How) is the participant interacting/ communicating with the employees? & that people find us more likable again, that's been our theme. To build up a bit of closeness. We made a video series where we were interviewed. So a few teammates, me, that they so on the physical, so we had nine interviews. (P4) &
4.6
%\ref{sec:res:employees} 
& 69\\

\rowcolor[HTML]{EFEFEF}Usable Security \& Security Friction & Are usability aspects of security considered by the participant or other stakeholders? Are negative side effects of security/awareness/training considered? & So our CISO sits in there as an example, the head of IT, was still a board member on that UX team before. It was the corporate communications among others in this UX team (P5) & 
4.6.1
%\ref{results:securityfriction} 
& 62 \\

Groups of Employees & Which groups of employees is the awareness for (\eg, developers, cooks, blue color workers)? & Of course, an IT department has a few more additional training courses than a Business, for example. And Business has different training than HR, for example. & 
4.2.3
%\ref{results:whatInformsAwareness} 
& 46 \\


 \rowcolor[HTML]{EFEFEF}Effort Required & Effort (for security/for training) that is required from the employees.& "Hey, my people don't have that kind of time. My people might be prosecutors, they don't have time for a 1.5-hour training, they only have time for an e-learning." Then, of course, they can just get the e-learning. (P7) &
 4.6
%\ref{sec:res:employees} 
 & 40 \\

Feedback \& Requests & Employees give feedback on awareness measures or request a change/new measure. & But but yeah, it's not really something we've been very good at, to be honest, is getting that feedback. (P15) & 
4.3.1, 4.3.2
%\ref{results:goal}, \ref{results:measuring} 
& 29 \\

\rowcolor[HTML]{EFEFEF}\textbf{Awareness} & - & - & -& - \\

What is (not) awareness? & Definition of Awareness (less of "What they do"?) & So for me, I would always reflect it as phishing. (P7) & 
4.3
%\ref{sec:results-whatisgood}
& 56 \\

\rowcolor[HTML]{EFEFEF}Topics & What are the awareness measures about? &Then, for example, I would plan such a campaign on Identity-Theft. (P2) & 
4.2.2
%\ref{results:topics} 
& 61\\

Good Product & What makes a good awareness product? & I need customizable so my preliminary requirement. (P12) & 
4.3.2, 4.4.1
%\ref{results:measuring}, \ref{results:vendors}
& 32\\

\rowcolor[HTML]{EFEFEF}\textbf{Role} & - & - &- & - \\

Collaboration \& Alliances & With whom do they work together in their everyday working routine? & We are also very much in touch with fraud management because it is simply a big issue in the bank. Exactly, so fraud, customer fraud. (P1) & 
4.5
%\ref{results:alliances}
& 79 \\

\rowcolor[HTML]{EFEFEF}Decisions \& Power & What kinds of decisions do and can the participants make in their job& But it can always be that one boss, so the CISO, then comes and says, hey like we might have to do that thematically necessary now because it's in other boards still within where we have to do that? (P4) & 
4.5
%\ref{results:power} 
& 42 \\

Tasks \& Responsibilities & What are the concrete tasks of the participants? & these are the videos, these are presentations that I prepare and PowerPoint presentations. (P8) & 
4.5
%\ref{results:alliances} 
& 129 \\

 \hline\hline
\end{tabular}
\end{table*}
